Theoretically Better and Numerically Faster Distributed Optimization with Smoothness-Aware Quantization Techniques

To address the high communication costs of distributed machine learning, a large body of work has been devoted in recent years to designing various compression strategies, such as sparsification and quantization, and optimization algorithms capable of using them. Recently, Safaryan et al. (2021) pioneered a dramatically different compression design approach: they first use the local training data to form local smoothness matrices and then propose to design a compressor capable of exploiting the smoothness information contained therein. While this novel approach leads to substantial savings in communication, it is limited to sparsification as it crucially depends on the linearity of the compression operator. In this work, we generalize their smoothness-aware compression strategy to arbitrary unbiased compression operators, which also include sparsification. Specializing our results to stochastic quantization, we guarantee significant savings in communication complexity compared to standard quantization. In particular, we prove that block quantization with $n$ blocks theoretically outperforms single block quantization, leading to a reduction in communication complexity by an $\mathcal{O}(n)$ factor, where $n$ is the number of nodes in the distributed system. Finally, we provide extensive numerical evidence with convex optimization problems that our smoothness-aware quantization strategies outperform existing quantization schemes as well as the aforementioned smoothness-aware sparsification strategies with respect to three evaluation metrics: the number of iterations, the total amount of bits communicated, and wall-clock time.

==> commands.tex <==
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\mathtoolsset{showmanualtags}
\usepackage{amsthm}
\usepackage{xcolor}
\usepackage{tabularx}
\usepackage{bbm}
\usepackage{todonotes}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{makecell}
\usepackage{subcaption}


\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\dmitry}[1]{\todo[inline]{\footnotesize Dmitry: #1}}
\newcommand{\peter}[1]{\todo[inline]{\footnotesize Peter: #1}}
\newcommand{\adil}[1]{\todo[inline]{\footnotesize Adil: #1}}
\newcommand{\as}[1]{{\color{green} #1}}
\newcommand{\asnote}[1]{\todo[color=green!]{#1}}

\allowdisplaybreaks[1]

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}


\newcommand{\AG}{\mathrm{AG}}

\newcommand{\prox}{\mathrm{prox}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\Comp}{\mathrm{Comp}}
\newcommand{\Comm}{\mathrm{Comm}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\lmax}{\lambda_{\max}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lminp}{\lambda_{\min}^+}
\newcommand{\sign}{\mathrm{sign}}

\newcommand{\bg}{\mathrm{D}}

\newcommand{\R}{\mathbb{R}}

\def\<#1,#2>{\langle #1,#2\rangle}

\newcommand{\Dotprod}[1]{\left\langle#1\right\rangle}


\newcommand{\norm}[1]{\|#1\|}
\newcommand{\sqn}[1]{\norm{#1}_2^2}
\newcommand{\Norm}[1]{\left\|#1\right\|}
\newcommand{\sqN}[1]{\Norm{#1}^2}
\newcommand{\vect}[1]{\begin{bmatrix*}[c]#1\end{bmatrix*}}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\infNorm}[1]{\Norm{#1}_{\infty}}


\newcommand{\cR}{\mathcal{R}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\sX}{{\mathsf E}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\Lag}{\mathcal{L}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\sqNP}[1]{\Norm{#1}^2_\mP}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mWp}{\mathbf{W}^{\dagger}}
\newcommand{\sqnw}[1]{\sqn{#1}_{\mWp}}
\newcommand{\eqdef}{\coloneqq}
\DeclareMathOperator*{\argmin}{arg\,min}

